Universally-Optimal Distributed Algorithms for Known Topologies

Many distributed optimization algorithms achieve existentially-optimal running times, meaning that there exists some pathological worst-case topology on which no algorithm can do better. Still, most networks of interest allow for exponentially faster algorithms. This motivates two questions: (1) What network topology parameters determine the complexity of distributed optimization? (2) Are there universally-optimal algorithms that are as fast as possible on every topology? We resolve these 25-year-old open problems in the known-topology setting (i.e., supported CONGEST) for a wide class of global network optimization problems including MST, $(1+\varepsilon)$-min cut, various approximate shortest paths problems, sub-graph connectivity, etc. In particular, we provide several (equivalent) graph parameters and show they are tight universal lower bounds for the above problems, fully characterizing their inherent complexity. Our results also imply that algorithms based on the low-congestion shortcut framework match the above lower bound, making them universally optimal if shortcuts are efficiently approximable. We leverage a recent result in hop-constrained oblivious routing to show this is the case if the topology is known -- giving universally-optimal algorithms for all above problems.

==> related-work.tex <==
%\section{Further Related Work}\label{sec:related-work}

\smallskip 
Probably the most well-studied optimization problem in the distributed message-passing literature, and the one that best illustrates the search for universal optimality, is the MST problem. We discuss some of the literature on this problem here in more detail.

\smallskip

The MST problem was first studied in a distributed setting in the seminal work of \citet*{gallager1983distributed}, who gave an $O(n\log n)$-time MST algorithm. This was later improved  by \citet{awerbuch1987optimal} to $O(n)$ time, which is existentially optimal, due $\Omega(n)$-diameter graphs.
\citet{garay1998sublinear}, advocating for more refined analysis, moved closer to the universal lower bound of $\Omega(D)$, giving an $\tilde{O}(D + n^{0.613})$-time algorithm. This was later improved to $\tilde{O}(D + \sqrt{n})$ \cite{kutten1998fast}, with example networks proving this bound is also existentially optimal given by \citet{peleg2000near}.
These networks were then used to prove lower bounds for approximate MST by \citet{elkin2006unconditional}, and many other problems by \citet{dassarma2012distributed}. 
The existentially-optimal $\tO(D+\sqrt{n})$ upper bound was obtained by numerous algorithms over the years \cite{elkin2006faster,pandurangan2017time,elkin2017simple}, including using the shortcuts framework in \cite{ghaffari2016distributed}.

\medskip



\noindent\textbf{Restricted topologies.} The above works have motivated much work on studying other graph parameters which allow for improved running time for this problem. 
One example is restricting the diameter even further. 
For example, for graphs of diameter 1 (i.e., the congested clique model), a sequence of works \cite{lotker2003mst,hegeman2015toward,ghaffari2016mst} culminated in an $O(1)$-time algorithm \cite{jurdzinski2018mst}.
For higher diameter, \citet{lotker2006distributed}~gave an $O(\log n)$ algorithm for diameter-2 graphs, and $\tilde{\Omega}(\sqrt[3]{n})$ and $\tilde{\Omega}(\sqrt[4]{n})$ lower bounds for graphs of diameter 3 and 4, with  algorithms matching these bounds recently given by \cite{kitamura2019low} using the shortcuts framework of \cite{ghaffari2016distributed}. 
Indeed, the shortcuts framework has been the driving force behind numerous improved results for restricted graph families \cite{ghaffari2016distributed,haeupler2016low,haeupler2016near,haeupler2018minor,ghaffari2018new,ghaffari2017distributed,kitamura2019low,haeupler2018round}. 
For most of these results, the worst-case shortcut quality a graph in the graph family serves as an upper bound for these algorithms' running time. Our lower bounds imply that these algorithms are existentially optimal (for their respective graph families). Moreover, they hint\todo{no hinting. we have algorithms} that refined bounds can be obtained by one uniform algorithm, without having to design tailor-made algorithms for graph families of interest.


%All of these problems are by now known to be solvable using a polylogarithmic number of applications of part-wise aggregation
%\cite{ghaffari2016distributed,haeupler2018faster, dassarma2012distributed}.\todo{\small paste more}
%% (for verification problems, we outline this in \Cref{sec:verification}).
%Therefore, for graphs where part-wise aggregation is solvable in shortcuts quality time, $\tilde{O}(Q(G))$, these problems 
%are solvable in $\tilde{O}(Q(G))$ time. In this work we give strong evidence that this graph parameter is actually a universally-optimal bound for these problems.


%\medskip
%
%\noindent\textbf{Search for the Right Parameter.} Other refined bounds \cite[Section 1.3]{elkin2006faster}. "The main motivation for the result of"
%\cite{peleg2000distributed} distributed computing: a locality-sensitive approach.


\medskip
\noindent\textbf{Message Complexity.}
Another measure of message-passing algorithms is their \emph{message complexity}, i.e., the number of messages they send during their execution. 
\citet{awerbuch1990tradeoff} showed that any MST algorithm (under some conditions) in $m$-edge graphs must send $\Omega(m)$ messages---matched by many algorithms.
Whether existentially-optimal time and message complexities are achievable simultaneously was open, until a recent breakthrough of \citet{pandurangan2017time}, who gave a randomized algorithm achieving just that. This was then shown to be achievable deterministically, by \citet{elkin2017simple}, and then shown to be achievable within the shortcuts framework, in \cite{haeupler2018round}.
This leaves open the possibility of algorithms which have both universally-optimal time complexity, and optimal message complexity.

 
%Whether universally-optimal time complexity and message complexity are achievable simultaneously is, of course, unclear as of yet, as we do 
%In a recent brea
%
%Recent work has shown that both this optimal message complexity and $\tilde{O}(D+\sqrt{n})$ existentially-optimal running time are achievable \emph{simultaneously}, by a single algorithm \cite{pandurangan2017time,elkin2017simple,haeupler2018round}. In particular, such results are known to be achievable using an extension of the low-congestion shortcuts framework, implying optimal message complexity together with improved bounds for restricted graph classes \cite{haeupler2018round}. 
%Do we want to discuss sublinear in $m$ bounds? e.g.\cite{ghaffari2018distributed}.



%\medskip
%\noindent\textbf{Bounded-Diameter Graphs.} Another family of interest in which MST was studied is bounded-diameter graphs. In particular, \citet{lotker2006distributed}~gave an $O(\log n)$ algorithm for diameter-2 graphs, and $\tilde{\Omega}(\sqrt[3]{n})$ and $\tilde{\Omega}(\sqrt[4]{n})$ lower bounds for graphs of diameter 3 and 4, with  algorithms matching these bounds recently given by \cite{kitamura2019low} using the shortcuts framework of \cite{ghaffari2016distributed}. For graphs of diameter 1 (i.e., the congested clique model), a sequence of works \cite{lotker2003mst,hegeman2015toward,ghaffari2016mst} culminated in an $O(1)$-time algorithm \cite{jurdzinski2018mst}.

%\smallskip
%
%The \emph{shortcut quality} $Q(G)$ of a graph $G$ characterizes the worst possible partwise aggregation instance in $G$, and serves as a lower bound on the time to solve this problem using any shortcut-based strategy.
%Building on the framework of \cite{ghaffari2016distributed},
%this graph parameter $Q(G)$ underlies many results for distributed graph problems; it can be used to derive existentially-optimal algorithms for worst-case topologies \cite{ghaffari2016distributed}, and many improved algorithms for restricted topologies \cite{ghaffari2016distributed,haeupler2016low,haeupler2016near,haeupler2018minor,ghaffari2018new,ghaffari2017distributed,kitamura2019low,haeupler2018round}. By and large, these results for a family of graphs $\calF$ with $Q(\calF):=\max_{G\in \calF} Q(G)$ rely on the approach of \cite{ghaffari2016distributed} together with an $\tO(Q(\calF))$-time algorithms to compute $\tO(Q(\calF))$-quality shortcuts for connected partitions of graphs in $G$. 
%%Combined with the approach of \cite{ghaffari2016distributed}, this yields $\tO(Q(\calF))$-time algorithms for numerous problems in $\calF$.
%Indeed, for some families of graphs $\calF$, we even know how to compute $\tO(Q(G))$-quality shortcuts in $\tO(Q(G))$ time for every graph $G\in \calF$, leading to $\tO(Q(G))$-time algorithms for many problems in any $G\in \calF$ \cite{haeupler2016low}.

\medskip
\noindent\textbf{Universal Optimality.}
The notion of universal optimality (or \emph{instance-optimality}, as it is called in some fields) is a well-studied notion, and algorithms achieving this desired property are known in many computational models; these include aggregation algorithms for database systems \cite{fagin2003optimal}, shared memory distributed algorithms \cite{dwork1986knowledge}, 
geometric algorithms \cite{afshani2017instance}, and distribution testing and learning algorithms \cite{valiant2017automatic,valiant2016instance}. Indeed, the entire field of online algorithms and competitive analysis precisely concerns itself with notions of instance optimality.
For other models, instance-optimal algorithms were long sought after, but remain elusive. For example, one of the oldest open questions in computer science is the dynamic optimality conjecture of \citet{sleator1985self}, which states that splay trees are instance-optimal binary search trees.
%Closer to our problem, the closest result to a non-trivial instance-optimal message-passing algorithm is the $k$-broadcast algorithm of \citet{ghaffari2015distributed}, which is optimal among routing-based (supported CONGEST) algorithms.
%, and unfortunately requires additional preprocessing time (or alternatively, knowledge of the topology). 
%The challenge in achieving universally-optimal message-passing algorithms seems to be a lack of strong universal lower bounds to compare algorithms' running time to. 
%We present a family of universally-optimal algorithms for numerous problems, which are plausibly tight, thus making a step towards achieving universally-optimal message-passing algorithms.

%%% Local Variables:
%%% TeX-master: "main"
%%% End:

